A Gutzwiller Trace formula for Dirac Operators on a Stationary Spacetime

A Duistermaat-Guillemin-Gutzwiller trace formula for Dirac-type operators on a globally hyperbolic spatially compact stationary spacetime is achieved by generalising the recent construction by Strohmaier and Zelditch [Adv. Math. \textbf{376}, 107434 (2021)] to a vector bundle setting. We have analysed the spectrum of the Lie derivative with respect to a global timelike Killing vector field on the solution space of the Dirac equation and found that it consists of discrete real eigenvalues. The distributional trace of the time evolution operator has singularities at the periods of induced Killing flow on the manifold of lightlike geodesics. This gives rise to the Weyl law asymptotic at the vanishing period. A pivotal technical ingredient to prove these results is the Feynman propagator. In order to obtain a Fourier integral description of this propagator, we have generalised the classic work of Duistermaat and H\"{o}rmander [Acta Math. \textbf{128}, 183 (1972)] on distinguished parametrices for normally hyperbolic operators on a globally hyperbolic spacetime by propounding their microlocalisation theorem to a bundle setting. As a by-product of these analyses, another proof of the existence of Hadamard bisolutions for a normally hyperbolic operator (resp. Dirac-type operator) is reported.

==> conclusion.tex <==
% ============================= 
\chapter{Conclusion}
% ============================= 
% ============================= 
\section{Summary}
% ============================= 

% ============================= 
\section{Future scopes}
% ============================= 
A brief synopsis of this thesis will be presented in this chapter with possible extensions 
and open questions of an on going research. 
To start with, we have been able to prove that the ground state of the Dirac field on a static spacetime
satisfies the modular $\lp$-condition. 
Employing deformation argument, one can extend this result for any globally hyperbolic spacetime.  
\newline 



In the next level, the \mlp is used to estimate an upper bound for the modular entanglement 
for ground state over an arbitrary bipartite system separated by a nonzero distance $d$.  
We compute the scaling behavior of the modular entanglement for two limiting cases of $d$:  
(i) the long distance behavior ($ d \to \infty $), where the entanglement entropy exhibits exponential falloff, and  
(ii) the short distance behavior ($ d \to 0 $), where we have obtained a volume law. 
At present, it is not clear why our computation has been incapable of showing the celebrated 
area law~\cite{Chandran_Entropy2016} behavior. 
We suspect that the computation is too crude to capture the small $d$ physics, 
as indicated from the work of Hollands and Sanders. 
Considering static spacetime of the form $ \mf_{0} = \R^{1, 1} \times \varSigma $, 
where $\varSigma$ is a compact $ D - 2 $ dimensional spin spacetime, they obtained~\cite[Thm. 11]{HollandsSanders_2017} 
\begin{equation}
    \lim_{d \to 0} \REE (\omega_{0}) \leq - C \ln ( m d ) \frac{ | \partial \rA | }{ d^{D - 2} }.
\end{equation}
\newline 



We will close the dissertation by commenting on some further generalization and 
possible applications in other areas of physics. 
In the first instance, one could look for some specific spacetime geometries, interesting from physics point of view:
\begin{itemize}
    \item \textbf{Cosmological spacetime}:
    We live in an expanding universe, e.g., 
    the Friedmann-Lemaître-Robertson-Walker (FLRW) metric describes path-connected homogeneous, isotropic, and 
    expanding (contracting) universe, 
    the de Sitter metric models probable inflationary period. 
    Recently fermionic field has been proposed as  a candidate for inflation, dark energy and dark matter~\cite{Grams_CQG2014}.  
    Bell's inequality~\cite{Maldecena_FdP2016} and 
    von Neumann entanglement entropy for Klein-Gordon field~\cite{Iizuka_NuclPhysB2016}
    and Dirac field~\cite{Kanno_JHEP2017} 
    in de Sitter spacetime have been reported in contemporary. 
    Albeit entanglement entropy is computed for static spacetime in the present investigation, 
    our general framework has been developed for any globally hyperbolic spacetime, 
    and so it will be very interesting to study to entanglement entropy of fermions in such 
    cosmological spacetimes.
    
    \item \textbf{Black hole geometry}:
    As have mentioned already, microscopic derivation of Hawking-Bekenstein entropy is the historical motivation 
    to study entanglement entropy of quantum fields in curved spacetime 
    (see the review~\cite{Solodukhin_LivRevRelativity2011} and references therein for details). 
    The usual approach is to take black hole and its surrounding as a bipartite system 
    and look for von Neumann entanglement entropy when one is approaching very close 
    to the event horizon. 
    In our picture this can be accomplished by considering one of the regions $\rA$ or $\rB$ 
    equipped with a bifurcate Killing horizon and studying the behavior of entanglement entropy with their distance $d$. 
    Our framework explains the UV divergence behavior of when $d \to 0$, 
    and simultaneously accounts more realistic situation to probe interior of horizon 
    from far separated region (\ie $ d \to \infty $ case). 
\end{itemize}
The other analysis can be carried over possible generalization of states. 
We have presented the computation for ground state of Dirac field in static spacetime. 
One may also wish to look more general states relevant for physical applications:
\begin{itemize}
    \item \textbf{Thermal states}:
    The cosmic microwave background radiation implies that our universe evolve from a very hot thermal state 
    which reads a temperature around 2.7 Kelvin, at present. 
    To understand the role of entanglement from very early universe to present, and future, 
    it is utmost important to study the thermal states. 
    Since our general formalism has been developed for any quasifree states, 
    it will be a very interesting to investigate the thermal states.  
    
    \item \textbf{Nonquasifree states}: 
    Albeit quasifree states capture important states like ground state and thermal state, 
    but they are far away from containing all possible physically attractive states. 
    In fact, nonquasifree states are much less investigated due to their complexity, 
    and thus it will be itself an interesting area to explore with their entanglement behavior.  
    
    \item \textbf{Nonequilibrium states}: 
    The general theory of nonequilibrium states is still unknown. 
    A feasible case may be to study steady-state nonequilibrium states.  
    To best of our knowledge entanglement negativity for such states in conformal field theories 
    has been studied~\cite{Hoogeveen_Doyon_NuclPhysB_2015}.
    It will certain be interesting to look the results from rigorous operator algebraic 
    view point and extend for other entanglement measure, in particle the modular entanglement 
    studied in the present project. 
\end{itemize}
To end, we would like to investigate entanglement entropy for other field theories. 
After some experience from scalar and spinor quantum field theories, 
the obvious ambition is to look at gauge theories. 
They are physically very important since the standard model of particle physics is a Yang-Mills theory 
and thus indispensable to understand phenomenon from early universe cosmology to condensed matter system. 
Investigations of entanglement entropy on gauge theories has been is quite restrictive due to factorization 
problem of physical Hilbert space. 
Results have mostly achieved via replica trick (Section~\ref{sec: Euclidean_method}), 
often formulated first in lattice and then performing the continuum limit~\cite{Donnelly_CQG2014, Ghosh_JHEP2015, Soni_JHEP2016, Soni_JHEP2017}, 
Apart from the fundamental aspects, entanglement entropy may play the additional role of an order parameter 
for certain gauge theories.  
\begin{itemize}
    \item \textbf{Topological entanglement entropy}: 
    In quantum many-body system at zero temperature, a quantum phase transition may occur as a parameter 
    varies in the Hamiltonian of the system. 
    The correlation functions among the microscopic degrees of freedom have qualitatively different properties in the 
    two phases, but in some cases, the phase cannot be distinguished by any local order parameter. 
    At low energies, a $2+1$-dimensional system with a mass gap can exhibit topological order 
    and entanglement entropy of the ground state for the topological ordered phase provides global 
    information to characterize the order. 
    This kind of systems is quite common in condensed matter systems in two spatial dimensions, 
    for instance, the quantum Hall effect occurs in material whose low-energy theory is described by an 
    abelian Chern-Simons gauge theory. 
    The \textbf{topological entanglement entropy} $ E^{ \ms{\textrm{top}} } (\omega_{0}) $ 
    of a bipartite system in a compact Cauchy surface,
    is defined as the scale independent finite contribution 
    of the von Neumann entanglement entropy~\cite{KitaevPreskill_PRL2006}
    \begin{equation}
	\EEvN (\omega_{0}) = \alpha | \partial \Cauchy | - E^{ \ms{\textrm{top}} } (\omega_{0}), 
    \end{equation}
    where the coefficient $\alpha$, arising from short wavelength modes near the boundary, 
    is nonuniversal and UV divergent, 
    but $ E^{ \ms{\textrm{top}} } (\omega_{0}) $ is a nonnegative universal additive constant 
    equals to the logarithm of the total quantum dimensions of a particle.  
    This has been computed for several models and 
    we refer the reviews~\cite{Nishioka_JPA2009, Laflorenci_PR2016} for details.
    Recently similar notion has been captured for relative entanglement entropy in 
    operator algebraic setting~\cite[Prop. 4]{HollandsSanders_2017}. 
    
    \item \textbf{Confinement/deconfinement transition}: 
    One of the interesting applications of entanglement entropy can be the identification as an 
    order parameter for the confinement / deconfinement phase transition of gauge theories. 
    When we divide the Cauchy hypersurface $\Cauchy$ as a bipartition $ \rA \sqcup \rA' = \Cauchy $, 
    the entanglement entropy between the two regions measures the effective degrees of freedom at 
    the energy $1 / |\partial \rA|$. 
    Then in the confining gauge theory, the von Neumann entanglement entropy should become trivial 
    (approaches to a constant) as $ |\partial \rA| \to \infty $. 
    Computations have been performed via the holographic method (Section~\ref{sec: holographic_method}), 
    where certain strongly interacting (supersymmetric) quantum field theories  
    can be mapped to weakly coupled classical gravity theory. 
    For a status report, we refer the review~\cite{Nishioka_JPA2009}. 
    So far, it is unknown how to formulate nonperturbative quantum field theories, 
    unless one aims numerical lattice computation. 
    A pragmatic strategy can be to investigate relatively simple toy models which shares  
    similar features of confining gauge theories. 
    Schwinger model~\cite{Schwinger_PR1962} is one of such models which is exactly solvable 
    with fermion confinement and has been long used as a prototype of quantum chromodynamics.   
    One could take this as a starting point and study the entanglement entropy of corresponding state.  
\end{itemize}
% =========================================================================

